Exploiting network topology for large-scale inference of nonlinear reaction models

The development of chemical reaction models aids understanding and prediction in areas ranging from biology to electrochemistry and combustion. A systematic approach to building reaction network models uses observational data not only to estimate unknown parameters, but also to learn model structure. Bayesian inference provides a natural approach to this data-driven construction of models. Yet traditional Bayesian model inference methodologies that numerically evaluate the evidence for each model are often infeasible for nonlinear reaction network inference, as the number of plausible models can be combinatorially large. Alternative approaches based on model-space sampling can enable large-scale network inference, but their realization presents many challenges. In this paper, we present new computational methods that make large-scale nonlinear network inference tractable. First, we exploit the topology of networks describing potential interactions among chemical species to design improved "between-model" proposals for reversible-jump Markov chain Monte Carlo. Second, we introduce a sensitivity-based determination of move types which, when combined with network-aware proposals, yields significant additional gains in sampling performance. These algorithms are demonstrated on inference problems drawn from systems biology, with nonlinear differential equation models of species interactions.

==> introduction.tex <==
Detailed chemical reaction networks are a critical component of simulation tools in a wide range of applications, including combustion, catalysis, electrochemistry, and biology. In addition to being used as predictive tools, reaction network models can encode a mechanistic understanding of the processes under study. The development of reaction networks typically entails three tasks: the selection of participating species, the identification of species interactions (referred to as reactions), and the calibration of unknown parameter values. To this end, we are often faced with the challenge of comparing a combinatorially large number of reaction networks, each containing parameterized reaction rate models derived from physical principles.
% that describe a set of nonlinear differential equations. 
The ideas presented in this paper make large-scale Bayesian inference of network structure and parameters \textit{feasible} by exploiting essential aspects of network topology. A related notion, popular in systems biology \cite{Brown2003,Gutenkunst2007},
 is that of  ``sloppy models''---i.e., models where the available data are able to constrain only a few directions in the parameter space. Our work exploits an analogous sloppiness in the \emph{structure} of reaction networks to achieve large gains in the efficiency of network inference.  

A standard approach to building models is to postulate reaction networks and to compare them based on their ability to reproduce indirect system-level experimental data. Data-driven approaches to network learning involve defining a metric of fit, e.g., penalized least-squares, cross-validation, model evidence, etc., and selecting models that optimize this metric. As such, the development of models involves not only the identification of the best model structure, but also the estimation of underlying parameter values given available data. Bayesian inference provides a rigorous statistical framework for fusing data with prior knowledge to yield a full description of model and parameter uncertainties \cite{Gelman2004}. The application of Bayesian model inference to reaction networks, however, presents a significant computational challenge. Model discrimination in Bayesian analysis is based on computing model probabilities conditioned on available data, i.e., \textit{posterior} model probabilities. Formally, the posterior probability of a model $M_{m}$ is given by
\begin{align*}
p(M_{m} \vert {\mathcal{D}})=\frac{p(M_{m})p({\mathcal{D}} \vert M_{m})}{\sum_{m} p(M_{m})p({\mathcal{D}} \vert M_{m})},
\end{align*}
\noindent      
where
\begin{equation*}
p(\mathcal{D} \vert M_{m})=\int \cdots \int p(\mathcal{D} \vert {{k}_{m}}, M_m) p({{k}_{m}} \vert M_{m})d {{k}_{m}}
\end{equation*}
\noindent
is known as the model evidence, $p(M_{m})$ is the prior probability of model $M_{m}$, ${k_{m}}$ is the vector of parameters in model $M_{m}$, and ${\mathcal{D}}$ denotes the available data. A common approach to Bayesian model inference is to construct the candidate models $\{ M_m \}$ such that the prior and posterior on each ${{k}_{m}}$ are conjugate distributions, thereby making the calculation of individual model evidences analytically tractable. For instance, reaction network inference has been performed with network edge interactions represented by linear models or categorical distributions; both cases allow the specification of conjugate priors \cite{Friedman2000,Sachs2002}. %
Even in this simple setting where model evidences can be evaluated analytically and relatively cheaply, the combinatorial explosion of the number of networks, given species and their possible interactions, precludes direct enumeration of all models. \emph{Sampling} approaches have thus been used to infer such statistical models \cite{Ellis2008}. 

It is, however, widely believed that species interactions are more appropriately defined by the law of mass action, which gives the rate of an elementary chemical reaction (say $X+Y\rightarrow Z$) as the product of a reaction-specific rate constant $k$ with reactant concentrations $[X]$ and $[Y]$:
\begin{equation}
\text{Rate}=-k [X] [Y].
\label{massactionkineticsrate}
\end{equation}
%
%\todo{Shouldn't there be, in general, exponents on the reactant concentrations?}\todo{I added 'elementary' reaction}
Using the law of mass action to define reaction rates produces a system of ordinary differential equations (ODEs), such that the map from parameters (e.g., rate constants ${{k}_{n}}$) to observables (e.g., selected species concentrations) is typically nonlinear. ODE-based species interaction models have recently been incorporated into %network 
model inference frameworks \cite{Braman2013,Xu2010}. %These equations can be further embedded into differential equation models that describe convective and diffusive transport, surface interactions, and other physical phenomena that affect experimental observations. 
Rigorous computation of posterior model probabilities then requires numerical evaluation of a high-dimensional integral for each model.  A number of  Monte Carlo methods have been proposed for this purpose, but they are computationally taxing \cite{Chib2001,Gelman1998}. Alternative approaches such as Laplace approximations and, relatedly, the Bayesian information criterion are faster, but they involve potentially crude approximations of the posterior distribution \cite{Mackay2003,Schwarz1978}. And when the number of competing models becomes large, all of these methods become computationally {infeasible}.

Reaction network inference is particularly prone to this difficulty: instead of a few model hypotheses, one might start with a list of proposed reactions and form a collection of plausible models by considering all valid combinations of the proposed reactions. Across-model sampling \cite{Green2009} offers a useful solution in this setting. These sampling methods involve a Markov chain Monte Carlo (MCMC) algorithm that ``jumps'' between models to explore the joint posterior distribution over models and parameters. Posterior model probabilities are estimated by counting the number of times the sampler visits each model; direct evaluations of the evidence for each model are thus avoided. Efficient across-model sampling, however, is quite challenging: it requires the careful design of proposals for between-model moves. Many practical applications of across-model sampling have relied on pilot runs of within-model posterior sampling to characterize the relevant distributions
 % to get a rough idea of the posterior distribution 
before employing an across-model sampler, although a few more automated methods do exist \cite{Green2009}. 
%
%The use of ODE-based forward models oftentimes results in nonlinear parameter-observable dependency---network inference then has to be based on the computation of model evidence numerically. % Xu et al. applied Bayesian model inference with nonlinear ODEs for the elucidation of ERK signalling pathway \cite{Xu2010}. Braman et al.\ used Bayesian methodology for the comparison of syngas chemistry models \cite{Braman2013}.%
% However, the methods used for numerical computation of evidence are limited to applications with a small  number of hand-crafted models. 
 Large-scale network inference with nonlinear forward models, in particular, has seen relatively limited attention \cite{Galagali2015}.
%
 A notable effort from Oates \textit{et al.}\ \cite{Oates2012} applies Bayesian model selection to ODE models systematically generated from potential species interactions, using reversible-jump MCMC (a general across-model sampling method) to simultaneously sample network topologies and their underlying rate parameters. Their approach employs standard methods for nested models: when adding reactions, the prior distribution is used to propose new reaction rates, and when swapping reactions, previous rate parameter values are simply retained. 
%
% employed a mixture of moves between models that either add/delete or swap reactions. When adding/deleting reactions, they used the parameter priors as the proposal distributions.  For a swap move, they assigned the same values to the parameters added into the model as the ones that were removed.  
%
In general, however, the posterior distribution can deviate significantly from the prior, such that sampling from the prior yields poor across-model mixing. Further, with nonlinear forward models, the posterior distributions of common reaction parameters can differ across models, such that retaining parameter values during swap moves is not efficient.
%
%Yet conventional \todo{Kind of colloquial; what makes the Oates method ``vanilla?''}
% across-model sampling methods are generally known to perform poorly. \todo{Kind of a strong and overly general statement to make without at least providing some citations at the end of the sentence. Can we add a few?}
%
% \todo{Starting here, I think the argument loses steam and needs some reworking. If Oates2012 already applied across-model sampling with nonlinear ODE-based forward models, what is missing? What is the new contribution of our paper? Is it that we are making sampling over candidate network models more efficient?  We should answer this question appropriately and then state the specifics to make the essence of our contribution concrete, i.e., come to a punch line that makes clear what we actually do. In my mind, this is that we perform an online analysis of network structure to construct better across-model moves, i.e., more effective ways of navigating through the discrete model space. This analysis accounts for sensitivities at the discrete level---i.e., the notion that, given a particular network structure, the presence of certain reactions will have no impact on the observables---and at the continuous (parameter) level---i.e., that the observables are more sensitive to changes in certain combinations of rate parameters than others. Could say more here, or perhaps cast it differently. But we should say something precise and compelling in this final paragraph of the intro!}
% %

In this paper, we present new methods for % large-scale
 Bayesian inference of chemical reaction networks. The essence of our approach is to exploit \emph{sensitivities} resulting from network structure. In particular, our approach performs an online analysis of network structure to construct better across-model moves, i.e., more effective ways of navigating through the discrete model space. This analysis accounts for sensitivities at the discrete level---the notion that, given a particular network structure, the presence of certain reactions will have no impact on the observables---and sensitivities at the continuous (parameter) level---the notion that observables are more sensitive to changes in certain combinations of rate parameters than in others. The resulting algorithms make fully Bayesian inference of reaction networks feasible in new problem settings, where existing approaches may fail to characterize the posterior distribution altogether.

% We develop algorithms that exploit structural properties of chemical reaction networks to improve exploration of posteriors over a large number of reaction networks in comparison to existing methods. 

% my mind, this is that 

% We develop a network-aware across-modeling sampling algorithm that recognizes the effective networks being inferred and exploits this knowledge to design efficient parameter proposals for moves between models. This translates into superior sampling performance and low-variance posterior estimates. The recognition of effective networks also allows derandomization of some conditional expectations and thereby yields further variance reduction. Not all reactions in a network are equally important in influencing the observables. The identification of reactions that have a sharper impact on observables can be critical in designing improved across-model samplers. We develop a local sensitivity-based metric to identify key reactions and use this to develop better between-model move proposals for the reversible jump MCMC algorithm. 

% Combining the sensitivity-based proposal construction along with network-aware sampling produces a highly improved nonlinear network inference algorithm.

%There is a need for the development of efficient large-scale network inference methods that would allow a systematic comparison of a large number of networks, but one that incorporates nonlinear forward models emerging from ODE-based species interaction formulations. In this paper, we present methods that exploit network topology of species interactions for efficient large-scale Bayesian inference of nonlinear chemical reaction networks.

